Towards a Holistic Integration of Spreadsheets with Databases: A Scalable Storage Engine for Presentational Data Management

Spreadsheet software is the tool of choice for interactive ad-hoc data management, with adoption by billions of users. However, spreadsheets are not scalable, unlike database systems. On the other hand, database systems, while highly scalable, do not support interactivity as a first-class primitive. We are developing DataSpread, to holistically integrate spreadsheets as a front-end interface with databases as a back-end datastore, providing scalability to spreadsheets, and interactivity to databases, an integration we term presentational data management (PDM). In this paper, we make a first step towards this vision: developing a storage engine for PDM, studying how to flexibly represent spreadsheet data within a database and how to support and maintain access by position. We first conduct an extensive survey of spreadsheet use to motivate our functional requirements for a storage engine for PDM. We develop a natural set of mechanisms for flexibly representing spreadsheet data and demonstrate that identifying the optimal representation is NP-Hard; however, we develop an efficient approach to identify the optimal representation from an important and intuitive subclass of representations. We extend our mechanisms with positional access mechanisms that don't suffer from cascading update issues, leading to constant time access and modification performance. We evaluate these representations on a workload of typical spreadsheets and spreadsheet operations, providing up to 20% reduction in storage, and up to 50% reduction in formula evaluation time.

==> graphs/data_models/raw_results <==
"C:\Program Files\Java\jdk1.8.0_65\bin\java" -Didea.launcher.port=7533 "-Didea.launcher.bin.path=C:\Program Files (x86)\JetBrains\IntelliJ IDEA 2016.2\bin" -Dfile.encoding=UTF-8 -classpath "C:\Program Files\Java\jdk1.8.0_65\jre\lib\charsets.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\deploy.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\access-bridge-64.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\cldrdata.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\dnsns.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\jaccess.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\jfxrt.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\localedata.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\nashorn.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\sunec.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\sunjce_provider.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\sunmscapi.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\sunpkcs11.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\zipfs.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\javaws.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\jce.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\jfr.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\jfxswt.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\jsse.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\management-agent.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\plugin.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\resources.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\rt.jar;C:\Users\Mangesh\IdeaProjects\dataspread\out\production\dataspread;C:\Users\Mangesh\IdeaProjects\dataspread\libs\postgresql-9.4-1201.jdbc41.jar;C:\Users\Mangesh\IdeaProjects\dataspread\libs\kryo-4.0.0.jar;C:\Users\Mangesh\IdeaProjects\dataspread\libs\minlog-1.3.0.jar;C:\Users\Mangesh\IdeaProjects\dataspread\libs\objenesis-2.1.jar;C:\Users\Mangesh\IdeaProjects\dataspread\libs\reflectasm-1.10.1-shaded.jar;C:\Program Files (x86)\JetBrains\IntelliJ IDEA 2016.2\lib\idea_rt.jar" com.intellij.rt.execution.application.AppMain Testing
2016-08-22 16:02:50 INFO   Testing main Testing started
2016-08-22 16:02:50 INFO   DBHandler connectDB Connected to Database
2016-08-22 16:02:51 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_01_rom
2016-08-22 16:03:05 INFO   Testing selectRange Select region  at random position Time taken(ms) = 135.17
2016-08-22 16:03:05 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_02_rom
2016-08-22 16:03:21 INFO   Testing selectRange Select region  at random position Time taken(ms) = 164.59
2016-08-22 16:03:21 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_05_rom
2016-08-22 16:03:41 INFO   Testing selectRange Select region  at random position Time taken(ms) = 197.54
2016-08-22 16:03:41 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_1_rom
2016-08-22 16:04:02 INFO   Testing selectRange Select region  at random position Time taken(ms) = 209.2
2016-08-22 16:04:02 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_2_rom
2016-08-22 16:04:25 INFO   Testing selectRange Select region  at random position Time taken(ms) = 228.16
2016-08-22 16:04:25 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_4_rom
2016-08-22 16:04:50 INFO   Testing selectRange Select region  at random position Time taken(ms) = 250.49
2016-08-22 16:04:50 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_6_rom
2016-08-22 16:05:18 INFO   Testing selectRange Select region  at random position Time taken(ms) = 279.18
2016-08-22 16:05:18 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_8_rom
2016-08-22 16:05:51 INFO   Testing selectRange Select region  at random position Time taken(ms) = 324.72
2016-08-22 16:05:51 INFO   Testing testUpdateOperations Table name = f_10000000_100_1_0_rom
2016-08-22 16:06:30 INFO   Testing selectRange Select region  at random position Time taken(ms) = 391.07
2016-08-22 16:06:30 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_01_rcv
2016-08-22 16:06:34 INFO   Testing selectRange Select region  at random position Time taken(ms) = 43.46
2016-08-22 16:06:34 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_02_rcv
2016-08-22 16:06:39 INFO   Testing selectRange Select region  at random position Time taken(ms) = 44.91
2016-08-22 16:06:39 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_05_rcv
2016-08-22 16:06:44 INFO   Testing selectRange Select region  at random position Time taken(ms) = 55.97
2016-08-22 16:06:45 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_1_rcv
2016-08-22 16:06:58 INFO   Testing selectRange Select region  at random position Time taken(ms) = 133.54
2016-08-22 16:06:58 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_2_rcv
2016-08-22 16:07:14 INFO   Testing selectRange Select region  at random position Time taken(ms) = 164.86
2016-08-22 16:07:15 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_4_rcv
2016-08-22 16:07:38 INFO   Testing selectRange Select region  at random position Time taken(ms) = 232.78
2016-08-22 16:07:38 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_6_rcv
2016-08-22 16:08:07 INFO   Testing selectRange Select region  at random position Time taken(ms) = 293.61
2016-08-22 16:08:07 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_8_rcv
2016-08-22 16:08:42 INFO   Testing selectRange Select region  at random position Time taken(ms) = 346.68
2016-08-22 16:08:42 INFO   Testing testUpdateOperations Table name = f_10000000_100_1_0_rcv
2016-08-22 16:09:23 INFO   Testing selectRange Select region  at random position Time taken(ms) = 410.81
2016-08-22 16:09:23 INFO   Testing main All Tests Done



2016-08-22 16:17:26 INFO   DBHandler connectDB Connected to Database
2016-08-22 16:17:27 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_01_rom
2016-08-22 16:17:34 INFO   Testing updateRectangular Update Dense region  at random position Time taken(ms) = 76.07
2016-08-22 16:17:35 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_02_rom
2016-08-22 16:17:42 INFO   Testing updateRectangular Update Dense region  at random position Time taken(ms) = 73.53
2016-08-22 16:17:42 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_05_rom
2016-08-22 16:17:50 INFO   Testing updateRectangular Update Dense region  at random position Time taken(ms) = 77.15
2016-08-22 16:17:50 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_1_rom
2016-08-22 16:17:58 INFO   Testing updateRectangular Update Dense region  at random position Time taken(ms) = 78.85
2016-08-22 16:17:58 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_2_rom
2016-08-22 16:18:07 INFO   Testing updateRectangular Update Dense region  at random position Time taken(ms) = 89.33
2016-08-22 16:18:07 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_4_rom
2016-08-22 16:18:16 INFO   Testing updateRectangular Update Dense region  at random position Time taken(ms) = 96.21
2016-08-22 16:18:17 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_6_rom
2016-08-22 16:18:29 INFO   Testing updateRectangular Update Dense region  at random position Time taken(ms) = 128.23
2016-08-22 16:18:29 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_8_rom
2016-08-22 16:18:43 INFO   Testing updateRectangular Update Dense region  at random position Time taken(ms) = 139.13
2016-08-22 16:18:43 INFO   Testing testUpdateOperations Table name = f_10000000_100_1_0_rom
2016-08-22 16:18:57 INFO   Testing updateRectangular Update Dense region  at random position Time taken(ms) = 132.03
2016-08-22 16:18:57 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_01_rcv
2016-08-22 16:19:08 INFO   Testing updateRectangular Update Dense region  at random position Time taken(ms) = 114.79
2016-08-22 16:19:08 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_02_rcv
2016-08-22 16:19:20 INFO   Testing updateRectangular Update Dense region  at random position Time taken(ms) = 120.16
2016-08-22 16:19:20 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_05_rcv
2016-08-22 16:19:32 INFO   Testing updateRectangular Update Dense region  at random position Time taken(ms) = 116.08
2016-08-22 16:19:32 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_1_rcv
2016-08-22 16:19:44 INFO   Testing updateRectangular Update Dense region  at random position Time taken(ms) = 118.68
2016-08-22 16:19:44 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_2_rcv
2016-08-22 16:19:56 INFO   Testing updateRectangular Update Dense region  at random position Time taken(ms) = 121.1
2016-08-22 16:19:56 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_4_rcv
2016-08-22 16:20:09 INFO   Testing updateRectangular Update Dense region  at random position Time taken(ms) = 130.02
2016-08-22 16:20:09 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_6_rcv
2016-08-22 16:20:24 INFO   Testing updateRectangular Update Dense region  at random position Time taken(ms) = 147.22
2016-08-22 16:20:24 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_8_rcv
2016-08-22 16:20:40 INFO   Testing updateRectangular Update Dense region  at random position Time taken(ms) = 156.23
2016-08-22 16:20:40 INFO   Testing testUpdateOperations Table name = f_10000000_100_1_0_rcv
2016-08-22 16:20:56 INFO   Testing updateRectangular Update Dense region  at random position Time taken(ms) = 160.8
2016-08-22 16:20:56 INFO   Testing main All Tests Done




"C:\Program Files\Java\jdk1.8.0_65\bin\java" -Didea.launcher.port=7533 "-Didea.launcher.bin.path=C:\Program Files (x86)\JetBrains\IntelliJ IDEA 2016.2\bin" -Dfile.encoding=UTF-8 -classpath "C:\Program Files\Java\jdk1.8.0_65\jre\lib\charsets.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\deploy.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\access-bridge-64.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\cldrdata.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\dnsns.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\jaccess.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\jfxrt.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\localedata.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\nashorn.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\sunec.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\sunjce_provider.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\sunmscapi.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\sunpkcs11.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\ext\zipfs.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\javaws.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\jce.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\jfr.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\jfxswt.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\jsse.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\management-agent.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\plugin.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\resources.jar;C:\Program Files\Java\jdk1.8.0_65\jre\lib\rt.jar;C:\Users\Mangesh\IdeaProjects\dataspread\out\production\dataspread;C:\Users\Mangesh\IdeaProjects\dataspread\libs\postgresql-9.4-1201.jdbc41.jar;C:\Users\Mangesh\IdeaProjects\dataspread\libs\kryo-4.0.0.jar;C:\Users\Mangesh\IdeaProjects\dataspread\libs\minlog-1.3.0.jar;C:\Users\Mangesh\IdeaProjects\dataspread\libs\objenesis-2.1.jar;C:\Users\Mangesh\IdeaProjects\dataspread\libs\reflectasm-1.10.1-shaded.jar;C:\Program Files (x86)\JetBrains\IntelliJ IDEA 2016.2\lib\idea_rt.jar" com.intellij.rt.execution.application.AppMain Testing
2016-08-22 16:48:31 INFO   Testing main Testing started
2016-08-22 16:48:31 INFO   DBHandler connectDB Connected to Database
2016-08-22 16:48:32 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_01_rom
2016-08-22 16:48:39 INFO   Testing deleteRange Delete region  at random position Time taken(ms) = 68.33
2016-08-22 16:48:39 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_02_rom
2016-08-22 16:48:49 INFO   Testing deleteRange Delete region  at random position Time taken(ms) = 105.1
2016-08-22 16:48:49 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_05_rom
2016-08-22 16:49:08 INFO   Testing deleteRange Delete region  at random position Time taken(ms) = 180.11
2016-08-22 16:49:08 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_1_rom
2016-08-22 16:49:43 INFO   Testing deleteRange Delete region  at random position Time taken(ms) = 350.11
2016-08-22 16:49:43 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_2_rom
2016-08-22 16:51:24 INFO   Testing deleteRange Delete region  at random position Time taken(ms) = 1013.9
2016-08-22 16:51:24 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_4_rom
2016-08-22 16:56:55 INFO   Testing deleteRange Delete region  at random position Time taken(ms) = 3311.77
2016-08-22 16:56:55 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_6_rom
2016-08-22 16:57:29 INFO   Testing deleteRange Delete region  at random position Time taken(ms) = 339.93
2016-08-22 16:57:30 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_8_rom
2016-08-22 16:58:03 INFO   Testing deleteRange Delete region  at random position Time taken(ms) = 336.17
2016-08-22 16:58:04 INFO   Testing testUpdateOperations Table name = f_10000000_100_1_0_rom
2016-08-22 16:58:46 INFO   Testing deleteRange Delete region  at random position Time taken(ms) = 426.82
2016-08-22 16:58:46 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_01_rcv
2016-08-22 16:58:52 INFO   Testing deleteRange Delete region  at random position Time taken(ms) = 55.19
2016-08-22 16:58:52 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_02_rcv
2016-08-22 16:58:58 INFO   Testing deleteRange Delete region  at random position Time taken(ms) = 59.8
2016-08-22 16:58:58 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_05_rcv
2016-08-22 16:59:04 INFO   Testing deleteRange Delete region  at random position Time taken(ms) = 55.59
2016-08-22 16:59:04 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_1_rcv
2016-08-22 16:59:18 INFO   Testing deleteRange Delete region  at random position Time taken(ms) = 139.64
2016-08-22 16:59:18 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_2_rcv
2016-08-22 16:59:33 INFO   Testing deleteRange Delete region  at random position Time taken(ms) = 150.65
2016-08-22 16:59:33 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_4_rcv
2016-08-22 16:59:57 INFO   Testing deleteRange Delete region  at random position Time taken(ms) = 236.92
2016-08-22 16:59:57 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_6_rcv
2016-08-22 17:00:19 INFO   Testing deleteRange Delete region  at random position Time taken(ms) = 221.09
2016-08-22 17:00:19 INFO   Testing testUpdateOperations Table name = f_10000000_100_0_8_rcv
2016-08-22 17:00:47 INFO   Testing deleteRange Delete region  at random position Time taken(ms) = 278.37
2016-08-22 17:00:47 INFO   Testing testUpdateOperations Table name = f_10000000_100_1_0_rcv
2016-08-22 17:01:22 INFO   Testing deleteRange Delete region  at random position Time taken(ms) = 354.81
2016-08-22 17:01:22 INFO   Testing main All Tests Done


2016-08-23 08:48:05 INFO   Testing main Testing started
2016-08-23 08:48:05 INFO   DBHandler connectDB Connected to Database
2016-08-23 08:48:06 INFO   Testing testUpdateOperations Table name = f_10000000_100_1_0_rom
2016-08-23 08:48:26 INFO   Testing selectRange Select region  at random position Time taken(ms) = 201.31
2016-08-23 08:48:26 INFO   Testing testUpdateOperations Table name = f_10000000_80_1_0_rom
2016-08-23 08:48:43 INFO   Testing selectRange Select region  at random position Time taken(ms) = 165.75
2016-08-23 08:48:43 INFO   Testing testUpdateOperations Table name = f_10000000_60_1_0_rom
2016-08-23 08:48:57 INFO   Testing selectRange Select region  at random position Time taken(ms) = 141.6
2016-08-23 08:48:57 INFO   Testing testUpdateOperations Table name = f_10000000_40_1_0_rom
2016-08-23 08:49:07 INFO   Testing selectRange Select region  at random position Time taken(ms) = 100.82
2016-08-23 08:49:08 INFO   Testing testUpdateOperations Table name = f_10000000_20_1_0_rom
2016-08-23 08:49:17 INFO   Testing selectRange Select region  at random position Time taken(ms) = 95.28
2016-08-23 08:49:17 INFO   Testing testUpdateOperations Table name = f_10000000_10_1_0_rom
2016-08-23 08:49:27 INFO   Testing selectRange Select region  at random position Time taken(ms) = 96.47
2016-08-23 08:49:27 INFO   Testing testUpdateOperations Table name = f_10000000_100_1_0_rcv
2016-08-23 08:49:49 INFO   Testing selectRange Select region  at random position Time taken(ms) = 224.66
2016-08-23 08:49:50 INFO   Testing testUpdateOperations Table name = f_10000000_80_1_0_rcv
2016-08-23 08:50:08 INFO   Testing selectRange Select region  at random position Time taken(ms) = 187.06
2016-08-23 08:50:08 INFO   Testing testUpdateOperations Table name = f_10000000_60_1_0_rcv
2016-08-23 08:50:24 INFO   Testing selectRange Select region  at random position Time taken(ms) = 159.91
2016-08-23 08:50:25 INFO   Testing testUpdateOperations Table name = f_10000000_40_1_0_rcv
2016-08-23 08:50:39 INFO   Testing selectRange Select region  at random position Time taken(ms) = 146.51
2016-08-23 08:50:39 INFO   Testing testUpdateOperations Table name = f_10000000_20_1_0_rcv
2016-08-23 08:50:52 INFO   Testing selectRange Select region  at random position Time taken(ms) = 126.59
2016-08-23 08:50:52 INFO   Testing testUpdateOperations Table name = f_10000000_10_1_0_rcv
2016-08-23 08:51:04 INFO   Testing selectRange Select region  at random position Time taken(ms) = 119.51
2016-08-23 08:51:04 INFO   Testing main All Tests Done


2016-08-23 10:55:28 INFO   Testing testUpdateOperations Table name = f_10000_100_1_0_rom
2016-08-23 10:55:36 INFO   Testing selectRange Select region  at random position Time taken(ms) = 71.88
2016-08-23 10:55:36 INFO   Testing testUpdateOperations Table name = f_100000_100_1_0_rom
2016-08-23 10:55:46 INFO   Testing selectRange Select region  at random position Time taken(ms) = 108.13
2016-08-23 10:55:47 INFO   Testing testUpdateOperations Table name = f_1000000_100_1_0_rom
2016-08-23 10:56:01 INFO   Testing selectRange Select region  at random position Time taken(ms) = 144.2
2016-08-23 10:56:01 INFO   Testing testUpdateOperations Table name = f_10000000_100_1_0_rom
2016-08-23 10:56:20 INFO   Testing selectRange Select region  at random position Time taken(ms) = 186.24
2016-08-23 10:56:20 INFO   Testing testUpdateOperations Table name = f_10000_100_1_0_rcv
2016-08-23 10:56:28 INFO   Testing selectRange Select region  at random position Time taken(ms) = 86.26
2016-08-23 10:56:29 INFO   Testing testUpdateOperations Table name = f_100000_100_1_0_rcv
2016-08-23 10:56:41 INFO   Testing selectRange Select region  at random position Time taken(ms) = 125.36
2016-08-23 10:56:41 INFO   Testing testUpdateOperations Table name = f_1000000_100_1_0_rcv
2016-08-23 10:56:55 INFO   Testing selectRange Select region  at random position Time taken(ms) = 134.99
2016-08-23 10:56:55 INFO   Testing testUpdateOperations Table name = f_10000000_100_1_0_rcv
2016-08-23 10:57:11 INFO   Testing selectRange Select region  at random position Time taken(ms) = 161.54

==> related_works.tex <==
\section{Related Work} \label{sec:related}

We described our vision for \system in an earlier demo paper~\cite{dbspread}. Our work draws on related work from multiple areas; we review papers in each of the areas, and describe how they relate to \system. We discuss 1) efforts that enhance the usability of databases, 2) those that attempt to merge the functionality of the two paradigms, but without a holistic integration, and 3) using Array and Graph based database management systems

% Previous work related to \system have proposed to enrich spreadsheets and relational databases with features from one another in three orthogonal directions: using spreadsheets to mimic the relational database functionalities, using databases to mimic spreadsheet functionalities, and exploiting the spreadsheet interface for querying data.

\stitle{1. Making databases more usable.} The database community has repeatedly lamented the lack of interface research \cite{lowell, jagadish_making_2007}. Much research has emerged in recent years, 
however, most of this research does not support direct data manipulation
in the manner spreadsheets do, rendering them unsuitable for interactive 
data management (as opposed to browsing or querying).
This includes recent work on gestural query and scrolling interfaces~\cite{idreos_dbtouch:_2013, mandel_gestural_2013, nandi_guided_2011, nandi_querying_2013, singh_skimmer:_2012}, 
visual query builders~\cite{abouzied_dataplay:_2012, catarci_visual_1997},
query sharing and recommendation tools~\cite{khoussainova_case_2009, chatzopoulou_query_2009, cetintemel_query_2013, khoussainova_snipsuggest:_2010},
schema-free databases~\cite{qian_crius:_2010},
schema summarization~\cite{yu_schema_2006},
and visual analytics tools~\cite{callahan_vistrails:_2006,mackinlay2007show, stolte2002polaris, gonzalez_google_2010}.

\stitle{2a. One way import of data from databases to spreadsheets.}
There are various mechanisms for 
importing data from databases to spreadsheets, and then
analyzing this data within the spreadsheet.
This approach is followed by Excel's Power BI tools, inluding Power Pivot~\cite{powerpivot},
with Power Query~\cite{powerquery} for exporting data
from databases and the web or deriving additional columns and Power View~\cite{powerquery}
to create presentations; 
and Zoho~\cite{zoho} and ExcelDB~\cite{exceldb} (on Excel), and
Blockspring~\cite{blockspring} (on Google Sheets~\cite{google-sheets})
enabling the
import from a variety of sources including the databases and the web.
Typically, the import is one-shot, with the data residing
in the spreadsheet from that point on, negating the scalability
benefits derived from the database.
Indeed, Excel 2013 specifies a limit of 1M records that can be analyzed
once imported, illustrating that the scalability benefits are lost;
Zoho specifies a limit of 0.5M records. Furthermore, the connection to the base data is lost: any modifications made at either end are not propagated.

\stitle{2b. One way export of operations from spreadsheets to databases.}
There has been some work on exporting spreadsheet operations
into database systems, such as the work from Oracle~\cite{witkowski_advanced_2005, witkowski_query_2005}
as well as startups 1010Data~\cite{1010data} and AirTable~\cite{airtable},
% removed two paeprs that were a demo and a conf version of a journal paper
to improve the performance of spreadsheets.
However, the database itself has no awareness of the existence of the
spreadsheet, making the integration superficial -- in particular, without
the database being aware of 
(a) the user window, it is cannot prioritize for
its execution over other computation (b) positional and ordering
aspects, it cannot support queries on that efficiently
(c) user operations on the front-end, e.g., inserts, deletes, 
moving formulae around, it cannot react to user events.
Indeed, the lack of awareness makes the integration one-shot, with
the current spreadsheet being exported to the database, with
no future interactions supported at either end:
thus, in a sense, the {\em interactivity} is lost.
% Other efforts in this space include
% that by Cunha et al.~\cite{cunha_spreadsheets_2009} to
% recognize functional dependencies in spreadsheets.
%


\stitle{2c. Using a spreadsheet to mimic a database.}
There has been efforts to use a spreadsheet
as an interface for posing traditional database queries. 
There is nothing preventing us from applying traditional database queries in our front-end as well.
One effort in this space is by Tyszkiewicz~\cite{tyszkiewicz_spreadsheet_2010},
who describes how to 
simulate database operations in a spreadsheet. However, this approach loses the scalability benefits of relational databases.
There has also been some isolated work augmenting spreadsheets by modifying 
the spreadsheet interface to support joins \eg Bakke et al.~\cite{bakke_spreadsheet-based_2011, bakke_schema-independent_2011}, by depicting relations
using a nested relational model.
Another effort is that by Liu et al.~\cite{liu_spreadsheet_2009},
where the goal is to use spreadsheet operations
to specify single-block SQL queries; 
this effort is essentially a replacement for visual query builders. The authors compare against visual query builders in their evaluation, as opposed to a holistic integration.
Recently, Google Sheets~\cite{google-sheets} has provided
the ability to use single-table SQL on its frontend, without 
availing of the scalability benefits of database integration.
Excel, with its Power Pivot and Power Query~\cite{powerquery} functionality
has made moves towards supporting SQL in the front-end, with
the same limitations. 

\stitle{3. Array and Graph database systems.} While there has been work on array-based databases, most of these systems do not support edits: for instance, data in a SciDB~\cite{Brown:2010:OSL:1807167.1807271} array is not update-able. SciDB supports an append-only, no-overwrite data model. Graph based database systems~\cite{Neo4j} scale naturally for graph-like queries \eg graph diameter computations, community detection. However, they do not semantically support operations such as joins, which are a commonplace in spreadsheets.

\if{0}

\stitle{Spreadsheets for Databases.} There has been prior work~\cite{tyszkiewicz2010spreadsheet} on demonstrating spreadsheets as relational database engines by utilizing spreadsheet formulae. This was attained by expressing operators of relational algebra by means of spreadsheet functions. While this achieves the expressivity of SQL, this approach doesn’t scale beyond spreadsheets with a few thousand rows of data. In contrast, in \system, our goal is to leverage the scalability of relational databases to support spreadsheets at scale, while retaining ad-hoc analysis capabilities and the ability to use arbitrary SQL.

\stitle{Databases for Spreadsheets.} {\em Query by Excel}~\cite{Witkowski:2003:SRO:872757.872767, Witkowski:2005:QE:1083592.1083733} extends SQL to mimic spreadsheet functionalities. Users can define typical spreadsheet like calculations over rows and columns by formulae, which gets translated into SQL. The computations are then performed by a relational database system. This approached achieves the scalable and parallel execution that databases provide. However, in addition to supporting operations on billions of records, \system also aids the ad-hoc tabular management and visualization capabilities provided by spreadsheets.

\stitle{Spreadsheets for Querying Data.} There is related work that provides an intuitive interface to query data~\cite{liu2009spreadsheet}. This paper proposes an extension of the set of spreadsheet functions by carefully designed database functions, whereby the user can speficy SQL queries in spreadsheet-like style. These additional operators were executed by a classical database engine eunning in the background. It was shown in~\cite{tyszkiewicz2010spreadsheet} that these functionalities can be achieved by the spreadsheet itself. The focus of this paper is to build an easy-to-use direct manipulation interface for non-technical users. In contrast, in \system, our goal is to retain the spreedsheet front-end that users are comfortable with, and efficiently support operations on billions of records.

With the goal to achieve the benefits of spreadsheets and relational databases while dealing with tabular data, our holistic unification strives to unify the notion of table in both systems.
Recent works have proposed to enrich spreadsheets and relational databases with features from one another in three orthogonal directions:
\begin{inparaenum}[\itshape a\upshape)]
\item Use of spreadsheets to mimic 
the relational database functionalities~\cite{tyszkiewicz2010spreadsheet}: Although this approach achieves expressivity of SQL, it is unable to leverage the scalability of databases. 
\item Use of databases to mimic spreadsheet functionalities~\cite{Witkowski:2003:SRO:872757.872767, Witkowski:2005:QE:1083592.1083733}: 
Although this approach achieves scalability of databases, it is does not support ad-hoc tabular management provided by spreadsheets. 
\item Use of spreadsheet interface for querying data~\cite{liu2009spreadsheet}.
This approach provides an intuitive interface to query data, but looses the expressivity of SQL as well as ad-hoc data management capabilities. 
\end{inparaenum}
\fi


==> sec-intro-old.tex <==
%!TEX root=DataSpread-models.tex

\section{Introduction} \label{sec:introduction}




\cut{
Databases lacks support of interactive user interfaces, relying on only batch-oriented command-line SQL for data manipulation and querying. Therefore, we saw a flurry of research in making db more usable and interactive, such as natural language or gesture-based database querying. In this paper, we draw inspiration from the most successful tabular interface/direct manipulation of tables --- spreadsheet. We study its key principles of direct manipulation of tables. We observe that these principles are fundamentally missing in relational databases and cannot be realized natively. Therefore, we develop how to enable these support of interactivity principles in databases to realize a spreadsheet-like interface.}

Spreadsheet software, from the pioneering VisiCalc~\cite{bricklin1984visicalc} to Microsoft Excel~\cite{msexcel}
and Google Sheets~\cite{googlesheets}, 
have found ubiquitous use in ad-hoc manipulation, management, and analysis of tabular data.
\st{
The billions who use spreadsheets take advantage of not only 
its ad-hoc nature and flexibility but also 
the
in-built statistical and visualization capabilities.
Spreadsheets cater to both novice and advanced users, spanning
businesses, universities, organizations, government,  and home.}
\begin{toreview}
Spreadsheets provide this functionality in a \emph{direct manipulation} 
interface~\cite{shneiderman_direct_1983,hutchins_direct_1985}
that caters to both novice as well as advanced
users, spanning businesses, schools, organizations, and home; spreadsheets have, in fact, been heralded as
the pioneering example of a direct manipulation interface.
\end{toreview}


Yet, this mass adoption of spreadsheets breeds new challenges. 
With the increasing sizes and complexities of data sets, as well as types of analyses, 
we see a frenzy to push the limits:
users are struggling to work with spreadsheet software on large datasets; 
they are trying to import large data sets into Excel (\eg billions of gene-gene interactions) and are failing at doing so.
% and are trying to 
% handle inconsistencies resulting from their own makeshift 
% strategies for collaboration (\eg by emailing back and forth), 
% with no data validation and error recovery mechanisms~\cite{powell_critical_2008, panko_what_1998}.
In response, \emph{spreadsheet softwares are stretching the size of data they can support}; 
\eg Excel has lifted its size limits from $65$k to $1$ million rows; 
\cut{
and added Power Query and PowerPivot~\cite{powerquery, powerpivot} to support one-shot import of data from databases in 2010;}
Google Sheets has expanded its size limit to $2$ million cells.
%As Section \ref{sec:spvsdb} will discuss, 
Despite these developments, these moves
are far from the kind of scale, \eg beyond memory limits, and functionality, \eg expressiveness,
that databases natively provide.

\begin{toreview}
On the other hand, relational databases, which are scalable and expressive by design, lack support of interactive user interfaces and rely on batch-oriented command-line SQL for data manipulation and querying. Therefore, we saw a flurry of research in making databases more usable and interactive, such as natural language~\cite{li2014constructing} or gesture-based database querying~\cite{jiang2013gesturequery}. 

This discussion raises the following question: {\bf\em can we holistically integrate relational databases and spreadsheets?}
That is;
\begin{inparaenum}[(i)]
	\item Can we provide the direct manipulation interface of spreadsheets, which so many
	end-users are so comfortable with, to manage tables stored within a relational databases? and
	\item Can we facilitate the spreadsheet software to leverage 
	the scalability of relational databases?
\end{inparaenum}

To address the first question, our challenge is to
efficiently support the principles of direct manipulation within databases. 
In this paper, we draw inspiration from spreadsheet software to identify and 
study a key principle of direct manipulation, \ie \emph{efficient spatial organization and addressing}. 
We observe that, since relational databases use an unordered ``set'' semantics, spatial organization
 and addressing is fundamentally missing and cannot be realized natively. 
This motivates the need for {\em positional indexes};
we develop and experiment with indexing mechanisms that
adapt traditional indexing schemes, to take position into account. 
The positional indexes enables us to impose a spatial notion
to the unordered ``set'' semantics provided by a relational database
thereby enabling us to present a relational table on a
spreadsheet interface that supports direct manipulation capabilities, 
\eg scrolling.
\end{toreview}  
Furthermore, we need to support spatial modifications to the spreadsheet.
Note that even a small spatial modification can be rather costly:
inserting a single row can impact
the row number of all subsequent rows.
How do we support such spatial modifications efficiently?
We develop {\em positional mapping} schemes that allow 
us to avoid the expensive computation that results from 
small modifications. 

\begin{toreview}
To support direct manipulation for relational tables we; 
\begin{inparaenum}[(i)]
\item Enable users to declare a spatial region on the front-end to correspond to a native table within the underlying database. 
\item Establish a bi-directional synchronization between the interface and the underlying table. That is, translate direct manipulation actions, \eg update of tuple values, reordering of tuples, into relational transactions and execute them on the underlying table and reflect any changes to the underlying table on the front-end.
\end{inparaenum}
This not only enables users to interact with relational tables in a direct manipulation way but also facilitates the table to be shared across multiple sheets.  
\end{toreview}

To address the second question, we need to efficiently
represent spreadsheet data within a database.
Spreadsheets rarely obey a 
fixed schema --- a user may paste several
``tabular'' or table-like regions within a spreadsheet, 
often interspersed with empty rows or columns.
Users may also embed formulae into spreadsheets, 
along with data.
This means that considering the entire sheet
as a single relation, with rows corresponding to rows
of the spreadsheet, and columns corresponding to columns
of the spreadsheet, can be very wasteful due to sparsity.
At the other extreme, we can consider only 
storing cells of the spreadsheet that are filled-in:
we can simply store a table with schema
(row number, column number, value):
this can be effective for highly sparse spreadsheets,
but is wasteful for dense spreadsheets with well-defined
tabular regions.
One can imagine hybrid representation schemes
that use both ``tabular'' and ``sparse'' representation schemes as
well or schemas that take access patterns, \eg via formulae, into account.
Furthermore, any tabular regions that correspond to native relational tables need to be persisted as-is within the database.
In this paper, we show that it is {\sc NP-Hard}
to identify the optimal storage representation, given a spreadsheet.
\msb{Can we quantify both storage and access as access cost?} 
Despite this wrinkle, we characterize a certain natural subset of representations
for which identifying the optimal one
is in fact, {\sc PTIME};
furthermore, we identify a collection of optimization
techniques that further reduce the computation complexity to
the point where the optimal representation can be identified 
in the time it takes to make a single pass over the data.



%supporting the pipeline of pre-processing and loading of data into a database. 

%We envision 


%That is, can we retain the direct data manipulation interface of spreadsheets that so many
%end-users are so comfortable with, while supporting that interface with
%a standard relational database, seamlessly leveraging
%the benefits of scalability and expressiveness?
%In addition, 
 
\begin{toreview}
By addressing the aforementioned challenges, 
we answer the question of whether {\em can we holistically integrate relational databases and spreadsheets
\underline{in the affirmative} in this paper}. 
We build a system, \system, that can not only provides a direct manipulation interface to relational databases, but also leverages the database to scale up the capabilities of spreadsheets 
\system uses a standard relational database as a backend
(currently PostgreSQL, but nothing ties us to that database),
with a web-based spreadsheet system~\cite{zk_spreadsheet}, which serves as a direct manipulation interface.
Leveraging the underlying database to optimize formulae evaluation is an interesting and important challenge but is beyond the scope of this paper.


\msb{TODO:
Add to technical section:
1. discussion about two way synchronization 
2. Add constraints to the optimization algorithms to enable users to describe a region. 
}
\end{toreview}

By using a standard relational database,
with no modifications to the underlying engine,
we can just seamlessly leverage improvements
to the database, 
while allowing the same data to be used by other
applications.
This allows a clean encapsulation and separation
of front-end and back-end code, and also admits
portability and a simpler design.
\system is fully functional --- the \system resources,
along with video and code can be found at \anon{[details redacted for double-blind purposes]}{\url{dataspread.github.io}}.
\anon{}{We demonstrated a primitive version of \system
at the VLDB conference last year~\cite{dataspread-demo}.}

% However, since databases and spreadsheets adopt very different
% ideologies, this integration is not trivial. In particular:
% \squishlist
% \item Databases natively use an unordered ``set'' semantics;
% how can databases be made to support an ordered semantics
% that is needed for spreadsheets?
% \item Spreadsheet users often scroll to arbitrary positions
% on a sheet; how do we efficiently support scrolling?
% \item Spreadsheet users often add, delete, or update
% large collections of rows at a certain position on the spreadsheet. 
% How can we efficiently
% support such positional updates?
% \item Spreadsheet users often make changes to the schema; they
% add, delete, or update columns. How can we support
% these changes efficiently?
% \item Spreadsheet users embed large numbers of formulae
% within spreadsheets; how do we capture these formulae within
% a database context, and efficiently execute them?
% \squishend

% \msb{Do we need to elaborate this a little more?}
% In this paper, we develop data models to optimally represent spreadsheet data within a database.
% Motived by the spreadsheet operational semantics, we introduce and develop three primitive data models corresponding to the extremities in terms of data representation. 
% We recognize that a single data model is unable to achieve optimality for an arbitrary spreadsheet instance. Hence, we introduce a hybrid data model which combines the primitives together to provide an optimal representation for a spreadsheet instance.
% We further demonstrate that putting together the primitive models is \mbox{NP-hard} for an arbitrary schema instance, and circumvent the challenge by proposing heuristics.
% Along with evaluating the performance of our data models we also evaluate the effectiveness of our heuristics.
% In addition, we augment our data models with auxiliary indices, that we call {\em positional indexing} structures. We then show further improvements in performance due to these positional indices.

 

While there have been many attempts at combining spreadsheets
and relational database functionality, ultimately, all of these
attempts fall short because they do not let spreadsheet users
perform ad-hoc data manipulation operations~\cite{witkowski_advanced_2005, witkowski_query_2005,liu_spreadsheet_2009}. 
Other work supports expressive and intuitive 
querying modalities without addressing scalability issues~\cite{bakke2016expressive, dataplay, gesturedb}, 
addressing an orthogonal problem. 
There have been efforts that enhance spreadsheets or databases without combining them~\cite{tyszkiewicz_spreadsheet_2010}. 
% Prior work that attempt to merge
% the functionality of the two paradigms did so without a holistic integration. 
Furthermore, while there has been work on array-based databases, most of these systems do not support edits: for instance, SciDB~\cite{Brown:2010:OSL:1807167.1807271} supports an append-only, no-overwrite data model. We describe related work in more detail in Section~\ref{sec:related}.




\stitle{Rest of the Paper.} The outline of the rest of 
the paper is as follows.

\squishlist
\item We begin with an empirical study of four real spreadsheet
datasets, plus an on-line user survey, targeted at {\em understanding
how spreadsheets are used for data analysis }
in Section~\ref{sec:empirical_study}. 
\item 
Then, in Section~\ref{sec:desiderata},
we introduce the notion of a 
{\em conceptual data model} for spreadsheet data, as well
as the set of operations we wish to support on
this data model.
\item In Section~\ref{sec:spreadsheet_representation},
we propose three {\em primitive data models}
for supporting the conceptual data model
within a database,
along with a {\em hybrid data model}
that combines the benefits of these primitive
data models.
We demonstrate that identifying the optimal
hybrid data model is {\sc NP-Hard},
but we can develop a {\sc PTIME} dynamic
programming algorithm that allows us to find
an approximately optimal solution.
\item Then, in Section~\ref{sec:positional_mapping}, 
we motivate the need for, and develop indexing solutions
for {\em positional mapping}---a method for reducing the impact of cascading updates
for inserts and deletes on all our data models.
\item We give a brief overview of the system architecture
from the perspective of our data models in Section \ref{sec:architecture}. We 
also describe how we seamlessly support standard relational operations in \system.
\item We perform experiments to evaluate our data models and positional 
mapping schemes in Section~\ref{sec:experiments}, 
and discuss related work in Section~\ref{sec:related}.
\squishend

